Definitions by Rewriting in the Calculus of Constructions

The main novelty of this paper is to consider an extension of the Calculus of Constructions where predicates can be defined with a general form of rewrite rules. We prove the strong normalization of the reduction relation generated by the beta-rule and the user-defined rules under some general syntactic conditions including confluence. As examples, we show that two important systems satisfy these conditions: a sub-system of the Calculus of Inductive Constructions which is the basis of the proof assistant Coq, and the Natural Deduction Modulo a large class of equational theories.

==> candidates.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% strong normalization

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\append{Strong normalization of admissible CAC's}
\label{app-sn}

The normalization proof is based on \cite{coquand90lf} which extends
to CC Tait and Girard's techniques of reducibility candidates. It is
done in three steps :

\begin{lst}{--}
  
\item In Subsection~\ref{subsec-cand}, we define the set of
  reducibility candidates. This is the domain of the forthcoming
  interpretations.

\item In Subsection~\ref{subsec-int}, \ref{subsec-const} and
  \ref{subsec-def}, we define an interpretation for each type. The key
  points are the interpretations of predicate symbols.

\item In Subsection~\ref{subsec-sn}, we prove that every term belongs
  to the interpretation of its type. The key point is the correctness
  of the computable closure.

\end{lst}












%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% reducibility candidates

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Reducibility candidates}
\label{subsec-cand}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\oO}{\o{\O}}
\newcommand{\oP}{\o{\P}}
\newcommand{\oK}{\o{\K}}
\newcommand{\oB}{\o{\mathbb{B}}}
\newcommand{\oX}{\o{\mathbb{X}}}
\newcommand{\oSN}{\o{\mathbb{SN}}}
\newcommand{\TY}{\mathbb{TY}}
\newcommand{\oTY}{\o{\TY}}

\newcommand{\GT}{_{\G \th T}}
\newcommand{\GTp}{_{\G \th T'}}
\newcommand{\GU}{_{\G \th U}}
\newcommand{\GUp}{_{\G \th U'}}
\newcommand{\GK}{_{\G \th K}}
\newcommand{\GB}{_{\G \th \B}}

\newcommand{\GpT}{_{\G' \th T}}
\newcommand{\GpU}{_{\G' \th U}}
\newcommand{\GpK}{_{\G' \th K}}
\newcommand{\GpB}{_{\G' \th \B}}

\newcommand{\GppU}{_{\G'' \th U}}

\newcommand{\DT}{_{\D \th T}}
\newcommand{\DTt}{_{\D \th T\t}}
\newcommand{\DxUVt}{_{\D \th (x:U\t)V\t}}
\newcommand{\DxUVpt}{_{\D \th (x:U\t)V'\t}}
\newcommand{\DXKVt}{_{\D \th (X:K\t)V\t}}
\newcommand{\DTtp}{_{\D \th T\t'}}
\newcommand{\DU}{_{\D \th U}}
\newcommand{\DUt}{_{\D \th U\t}}
\newcommand{\DUpt}{_{\D \th U'\t}}
\newcommand{\DVt}{_{\D \th V\t}}
\newcommand{\DK}{_{\D \th K}}
\newcommand{\DKt}{_{\D \th K\t}}
\newcommand{\DKtp}{_{\D \th K\t'}}
\newcommand{\Ds}{_{\D \th s}}
\newcommand{\Dsp}{_{\D \th s'}}
\newcommand{\DXt}{_{\D\th X\t}}
\newcommand{\DXtp}{_{\D\th X\t'}}
\newcommand{\DF}{_{\D\th F}}
\newcommand{\DC}{_{\D\th C}}
\newcommand{\DD}{_{\D\th D}}
\newcommand{\DE}{_{\D\th E}}
\newcommand{\DG}{_{\D\th G}}
\newcommand{\DDp}{_{\D\th D'}}

\newcommand{\DpTt}{_{\D' \th T\t}}
\newcommand{\DpU}{_{\D' \th U}}
\newcommand{\DpC}{_{\D' \th C}}
\newcommand{\DpD}{_{\D' \th D}}
\newcommand{\DpF}{_{\D' \th F}}
\newcommand{\DpUt}{_{\D' \th U\t}}
\newcommand{\DpKt}{_{\D' \th K\t}}
\newcommand{\DpVs}{_{\D' \th V\s}}
\newcommand{\DpXt}{_{\D'\th X\t}}

\newcommand{\DppU}{_{\D''\th U}}
\newcommand{\DppUt}{_{\D''\th U\t}}
\newcommand{\DppKt}{_{\D''\th K\t}}
\newcommand{\DppVs}{_{\D''\th V\s}}

\newcommand{\DpppU}{_{\D'''\th U}}

\newcommand{\Gp}{|_{\G'}}
\newcommand{\Dp}{|_{\D'}}
\newcommand{\Dpp}{|_{\D''}}
\newcommand{\Dppp}{|_{\D'''}}
\newcommand{\Dn}{|_{\D_n}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% term classes and type closures
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Among well-typed terms, we can distinguish three disjoint classes :

\begin{lst}{--}
\item the {\em kinds\,} are the terms $K$ such that $\G \th K:\B$,
\item the {\em predicates\,} are the terms $T$ such that $\G \th T:K$
  and $\G \th K:\B$,
\item the {\em objects\,} are the terms $t$ such $\G \th t:T$ and $\G
  \th T:\st$.
\end{lst}

Among kinds and predicates, we can also distinguish several disjoint
classes : the terms $T$ such that $\G \th T:s$, $\G \th T:\px{U}V$ or
$\G \th T:\pX{K}V$. Moreover, it is possible to define a well-founded
measure $\mu$ on kinds and predicates.

\newcommand{\SN}{\cS\cN}
\newcommand{\WN}{\cW\cN}
\newcommand{\CR}{\cC\cR}
\newcommand{\NF}{\cN\cF}

We let $\SN$ be the set of strongly normalizable terms, $\NF$ be the
set of terms in normal form, $\oTY$ be the set of closures $\G \TH T$
such that $T=\B$, $T$ is a kind or $T$ is a predicate, $\oT\GT$ be the
set of closures $\G' \TH t$ such that $\G \sle \G'$ and $\G' \th t:T$,
and $\oSN\GT = \{ \G' \TH t \in \oT\GT ~|~ t \in \SN \}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% reducibility candidates
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{dfn}[Reducibility candidates]
  A term is {\em neutral} if it is not an abstraction nor of the form
  $c(\vt)$ where $c$ is a constructor.
  
  By induction on $\mu(\G \TH T)$, we define the set $\cR\GT$ of {\em
    reducibility candidates\,} of type $\G \TH T$, the ordering
  relation $\le\GT$ on $\cR\GT$, the candidate $\top\GT \in \cR\GT$
  and the {\em restriction\,} $R\Gp \in \cR\GpT$ of a candidate $R \in
  \cR\GT$ to some environment $\G' \sge \G$.

\begin{lst}{\bu}
\item $T=\B$.
\begin{lst}{--}
\item $\cR\GB = \{ \oSN\GB \}$.
\item $R \le\GB R'$ iff $R = R'$.
\item $\top\GB = \oSN\GB$.
\item $R\Gp = R \cap \oT\GpB$.
\end{lst}

\item $\G \th T : s$.
\begin{lst}{--}
\item $\cR\GT$ is the set of $R \sle \oT\GT$ such that :
\begin{bfenumi}{R}
\item $R \sle \SN$,
\item if $\G' \TH t \in R$ and $t \a t'$ then $\G' \TH t' \in R$,
\item if $\G' \TH t \in \oT\GT$, $t$ is neutral and, for every reduct
  $t'$ of $t$, $\G' \TH t' \in R$, then $\G' \TH t \in R$,
\item if $\G' \TH t \in R$ and $\G' \sle \G''$ then $\G'' \TH t \in
  R$.
\end{bfenumi}
\item $R \le\GT R'$ iff $R \sle R'$.
\item $\top\GT = \oSN\GT$.
\item $R\Gp = R \cap \oT\GpT$.
\end{lst}

\item $\G \th T:\px{U}K$.
\begin{lst}{--}
\item $\cR\GT$ is the set of functions $R$ which, to $\G' \TH u \in
  \oT\GU$, associate an element of $\cR_{\G' \th (T~u)}$ such that :
\begin{bfenumi}{P}
\item if $u\a u'$ then $R(\G \TH u) = R(\G \TH u')$,
\item if $\G \sle \G'$ then $R(\G \TH u)\Gp = R(\G' \TH u)$.
\end{bfenumi}
\item $R \le\GT R'$ iff, for all $\G \TH u \in \oT\GU$, $R(\G \TH u)
  \le_{\G \th (T~u)} R'(\G \TH u)$.
\item $\top\GT(\G' \TH u) = \top_{\G' \th (T~u)}$.
\item $R\Gp = R|_{\oT\GpU}$.
\end{lst}

\item $\G \th T:\pX{K}L$.
\begin{lst}{--}
\item Let $\S\GK$ be the set of pairs $(\G' \TH U, S)$ such that $\G'
  \TH U \in \oT\GK$ and $S \in \cR\GpU$. $\cR\GT$ is the set of
  functions $R$ which, to $(\G' \TH U, S) \in \S\GK$, associate an
  element of $\cR_{\G' \th (T~U)}$ such that :
\begin{bfenumi}{P}
\item if $U\!\a\! U'$ then $R(\G \TH U, S) \!=\! R(\G \TH U', S)$,
\item if $\G \!\sle\! \G'$ then $R(\G \TH U, \!S)\Gp \!=\! R(\G' \TH
  U, \!S\Gp)$.
\end{bfenumi}
\item $R \le\GT R'$ iff, for all $(\G' \TH U, S) \in \S\GK$, $R(\G \TH
  U, S) \le_{\G \th (T~U)} R'(\G \TH U, S)$.
\item $\top\GT(\G' \TH U, S) = \top_{\G' \th (T~U)}$.
\item $R\Gp = R|_{\S\GpK}$.
\end{lst}

\end{lst}
\end{dfn}

We extended the definition given in \cite{coquand90lf} with the notion
of restriction and the property (P2) in order to show the correctness
of the interpretation of types.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% complete lattice
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\oa}{\o{a}}
\newcommand{\op}{\o{\phi}}
\renewcommand{\sb}{(S_b)\bb}

\begin{lem}
  $(\cR\GT,\le\GT)$ is a complete lattice.
\end{lem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% invariance by reduction
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lem}
\label{lem-red-cand}
If $T \ad^* T'$ then $\cR\GT = \cR\GTp$.
\end{lem}












%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 



==> interpretation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% interpretation of types

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Interpretation of types}
\label{subsec-int}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% definition of candidate assignment
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\domB}{\dom^\B}

\begin{dfn}[Candidate assignment]
  A {\em candidate assignment} $\xi$ is a mapping from $\XB$ to
  $\bigcup \,\{ \,\cR\DT ~|~ \D \TH T \in \oTY \}$. It is {\em
    compatible with\,} $(\t, \G, \D)$ where $\t : \G \a \D$ if, for
  all $X \in \domB(\G)$, $X\xi \in \cR\DXt$. The {\em restriction\,}
  $\xi\Gp$ of $\xi$ to $\G'$ is defined by $X(\xi\Gp) = (X\xi)\Gp$.
\end{dfn}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Dtx}[1][I]{_{\D,\t,\xi}^{#1}}
\newcommand{\Dtxp}[1][I]{_{\D,\t,\xi'}^{#1}}
\newcommand{\Dsx}{_{\D,\s,\xi}^I}
\newcommand{\Dsxp}{_{\D,\s,\xi'}^I}
\newcommand{\Dtpx}{_{\D,\t',\xi}^I}
\newcommand{\Dspx}{_{\D,\s',\xi}^I}
\newcommand{\Dspxp}[1][I]{_{\D,\s',\xi'}^{#1}}
\newcommand{\Dstxp}[1][I]{_{\D,\s\t,\xi'}^{#1}}
\newcommand{\Dspxpp}[1][I]{_{\D,\s',\xi''}^{#1}}

\newcommand{\Dptx}[1][I]{_{\D',\t,\xi\Dp}^{#1}}
\newcommand{\Dptxp}{_{\D',\t,\xi'\Dp}^I}
\newcommand{\Dptpxp}{_{\D',\t',\xi'\Dp}^I}
\newcommand{\Dptpx}[1][I]{_{\D',\t',\xi\Dp}^{#1}}
\newcommand{\Dpsx}{_{\D',\s,\xi\Dp}^I}
\newcommand{\Dpsxp}{_{\D',\s,\xi'\Dp}^I}
\newcommand{\Dpspx}{_{\D',\s',\xi\Dp}^I}
\newcommand{\Dptux}{_{\D',\t \cup \xu,\xi\Dp}^I}
\newcommand{\Dpspxp}{_{\D',\s',\xi'\Dp}^I}
\newcommand{\DptUSx}{_{\D',\t \cup \XU,\xi\Dp \cup \XS}^I}

\newcommand{\Dpptx}{_{\D'',\t,\xi\Dpp}^I}
\newcommand{\Dpptpx}[1][I]{_{\D'',\t',\xi\Dpp}^{#1}}
\newcommand{\Dpptpxp}{_{\D'',\t',\xi'\Dpp}^I}
\newcommand{\Dppsx}{_{\D'',\s,\xi\Dpp}^I}
\newcommand{\Dppsxp}{_{\D'',\s,\xi'\Dpp}^I}
\newcommand{\Dpptux}{_{\D'',\t \cup \xu,\xi\Dpp}^I}
\newcommand{\DpptUSx}{_{\D'',\t \cup \XU,\xi\Dpp \cup \XS}^I}

\newcommand{\Dpppsx}{_{\D''',\s,\xi\Dppp}^I}
\newcommand{\Dpppsxp}{_{\D'',\s,\xi'\Dpp}^I}

\newcommand{\J}[2]{\I{#1\!\th\!#2}}

\newcommand{\JG}[1]{\J{\G}{#1}}
\newcommand{\JGT}{\JG{T}}
\newcommand{\JGU}{\JG{U}}
\newcommand{\JGUp}{\JG{U'}}
\newcommand{\JGV}{\JG{V}}
\newcommand{\JGVp}{\JG{V'}}
\newcommand{\JGK}{\JG{K}}
\newcommand{\JGTp}{\JG{T'}}

\newcommand{\JGp}[1]{\J{\G'}{#1}}
\newcommand{\JGpV}{\JGp{V}}
\newcommand{\JGpVp}{\JGp{V'}}
\newcommand{\JGpU}{\JGp{U}}
\newcommand{\JGpT}{\JGp{T}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% definition of predicate symbol interpretation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In order to simplify the notations, we assume that, for all $F \in
\FB$ with $\tF = \pvxT \st$, $\n\vx = \at_F$, and write $F$ instead of
$[\vx:\vT]F(\vx)$.

\begin{dfn}{\bf(Predicate interpretation)}
  An {\em interpretation\,} for $F \in \FB$ is a function $I$ which,
  to any $\D$, associates an element of $\cR\DF$ such that :
\begin{lst}{}
\item [\bf(P3)] if $\D \sle \D'$ then $I\DF\Dp = I\DpF$.
\end{lst}
\end{dfn}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% definition of the interpretation schema
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{dfn}[Interpretation schema]
  The {\em interpretation\,} of a closure $\G\TH T \in \oTY$ w.r.t. an
  environment $\D$, a substitution $\t : \G \a \D$, a candidate
  assignment $\xi$ compatible with $(\t,\G,\D)$ and an interpretation
  $I_F$ for each symbol $F \in \FB$, is an element of $\cR\DTt$
  defined by induction on $T$ :

\begin{lst}{\bu}
\item $\JG{s}\Dtx = \oSN\Ds$,
  
\item $\JG{F(\vt)}\Dtx = I\DF(\va)$ where, if $\tF = \pvxT U$, $a_i =
  \D \TH t_i\t$ if $x_i \in \Xs$ and $a_i = (\D \TH t_i\t,
  \JG{t_i}\Dtx)$ if $x_i\in \XB$,

\item $\JG{X}\Dtx = X\xi$,
  
\item $\JG{\px{U}V}\Dtx = \{ \D' \TH t \in \oT\DxUVt ~|~ \all \D'' \TH
  u \in \JGU\Dptx$, $\D'' \TH (t~u) \in \J{\GxU}{V}\Dpptux \}$,
  
\item $\JG{\pX{K}V}\Dtx = \{ \D' \TH t \in \oT\DXKVt ~|~
  \all \D'' \TH U \in \JGK\Dptx$, $\D'' \th (t~U) \in \bigcap
  \,\{\, \J{\GXK}{V}\DpptUSx ~|~ S \IN \cR\DppU \} \}$,
  
\item $\JG{\lx{U}V}\Dtx$ is the function which, to $\D' \TH u \in
  \oT\DUt$, associates $\J{\GxU}{V}\Dptux$,
  
\item $\JG{\lX{K}V}\Dtx$ is the function which, to $(\D' \TH U, S) \in
  \S\DKt$, associates $\J{\GXK}{V}\DptUSx$,

\item $\JG{(V~u)}\Dtx = \JGV\Dtx(\D \TH u\t)$,
  
\item $\JG{(V~U)}\Dtx = \JGV\Dtx(\D \TH U\t, \JGU\Dtx)$.
\end{lst}
\end{dfn}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% correction of the interpretation schema
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The correctness of this definition follows from the following lemma.
The most delicate point is to prove that $\JG{\px{U}V}\Dtx$ satisfies
(R1) to (R4).

\begin{lem}[Interpretation correctness]
\label{lem-int-correct}
\hfill
\begin{enumalphai}
\item $\JGT\Dtx \in \cR\DTt$,
\item if $\t \a \t'$ then $\JGT\Dtx = \JGT\Dtpx$,
\item if $\D \sle \D'$ then $\JGT\Dtx\Dp = \JGT\Dptx$.
\end{enumalphai}
\end{lem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% candidate substitution lemma
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The interpretation enjoys the following property which is essential in
the definition of the interpretation for predicate symbols and in the
strong normalization proof.

\newcommand{\deux}{_{\G_2,\t_2,\xi_2}^I}
\newcommand{\deuxp}{_{\G_2',\t_2,\xi_2|_{\G_2'}}^I}
\newcommand{\deuxpu}{_{\G_2',\t_2 \cup \xu,\xi_2|_{\G_2'}}^I}
\newcommand{\deuxpp}{_{\G_2'',\t_2,\xi_2|_{\G_2''}}^I}
\newcommand{\deuxppu}{_{\G_2'',\t_2 \cup \xu,\xi_2|_{\G_2''}}^I}
\newcommand{\undeux}{_{\G_2,\t_1\t_2,\xi_{12}}^I}
\newcommand{\undeuxp}{_{\G_2',\t_1\t_2,\xi_{12}|_{\G_2'}}^I}
\newcommand{\undeuxpu}{_{\G_2',\t_1\t_2 \cup \xu,\xi_{12}|_{\G_2'}}^I}
\newcommand{\undeuxppu}{_{\G_2'',\t_1\t_2 \cup \xu,\xi_{12}|_{\G_2''}}^I}

\newcommand{\JT}{\J{\G_0}{T}\undeux}
\newcommand{\JTt}{\J{\G_1}{T\t_1}\deux}

\begin{lem}[Candidate substitution]
\label{lem-cand-subs}
Let $\G_0$, $\G_1$ and $\G_2$ be three valid environments, $\G_0 \th T
\in \oTY$, $\t_1 : \G_0 \a \G_1$ and $\t_2 : \G_1 \a \G_2$ be two
well-typed substitutions and $\xi_2$ be a candidate assignment
compatible with $(\t_2,\G_1,\G_2)$. Then, the candidate assignment
$\xi_{12}$ defined by $X\xi_{12} = \J{\G_1}{X\t_1}\deux$ is compatible
with $(\t_1\t_2,\G_0,\G_2)$ and $\JTt = \JT$.
\end{lem}














%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% interpretation of free predicate symbols

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Interpretation of free predicate symbols}
\label{subsec-const}

In this subsection, we assume given a function $J$ which, to any
interpretation $I$ for free predicate symbols, associates an
interpretation $J^I$ for defined predicate symbols.

We define the interpretation of free predicate symbols by
induction on $>_\cF$. Let $C \in \FC$ with $\tC = \pvxT \st$ and
assume that we have already defined an interpretation $H$ for the
symbols smaller than $C$.

$\cR\DC = \prod a_1 \IN A_1 \ldots \prod a_n \IN A_n. \cR_{\D_n \th
  C(\vt)}$ where :

\begin{lst}{--}
\item $a_i = \D_i \TH t_i$ and $A_i = \oT_{\D_{i-1} \th T_i\t}$ if
  $x_i \in \Xs$,
\item $a_i = (\D_i \TH t_i, S_i)$ and $A_i = \S_{\D_{i-1} \th T_i\t}$
  if $x_i \in \XB$,
\end{lst}

\noindent
$n=\at_C$, $\D_0 = \D$ and $\t = \vxt$.

Let $i$ such that $x_i \in \XB$. An interpretation $I$ for $D =_\cF C$
is {\em monotone\,} in its $i$-th argument if $I\DD(\va) \le
I\DD(\va')$ whenever $a_i' = (\D_i \TH t_i, S_i')$, $S_i \le S_i'$
and, for all $j\neq i$, $a_j = a_j'$.

We let $\cI_C^m$ be the set of interpretations for all $D =_\cF C$
that are monotone in their inductive arguments, and $\le_C$ be the
relation on $\cI_C^m$ defined by $I \le_C I'$ iff, for all $D =_\cF C$
and $\D$, $I\DD \le\DD I'\DD$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% complete lattice
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lem}
$(\cI_C^m,\le_C)$ is a complete lattice.
\end{lem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% definition of the interpretation for free predicate symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\CI}{^{C,I}}

\begin{dfn}{\bf(Interpretation of free predicate symbols)}
  Let $\vp\CI\DD(\va)$ be the set of $\D' \TH u \in \oSN_{\D_n \th
    D(\vt)}$ such that if $u$ reduces to a term of the form $d(\vu)$
  with $\td = \pvyU D(\vv)$ then, for all $i \in \acc(d)$, $\D' \TH
  u_i \in \J{\vy:\vU}{U_i}\Dptx[L \cup J^L]$ where $\t = \vyu$, $L = H
  \cup I$ and, for all $Y \in \FVB(U_i)$, $Y\xi = S_{\i_Y}$.
\end{dfn}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% well-definedness of the interpretation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lem}
  $\vp^C$ is a monotone application over $\cI_C^m$.
\end{lem}

  There are several things to prove :

\begin{lst}{--}
\item $\vp^C\DD$ belongs to $\cR\DD$ and satisfies the properties (P1)
  to (P3),
\item $\vp\CI$ is monotone in its inductive arguments,
\item $\vp^C$ is monotone.
\end{lst}

We just give some indications on how to prove the monotonicity of
$\vp^C$. Proving that $\vp\CI$ is monotone in its inductive arguments
uses the same kind of arguments. Let $I, I' \in \cI_C$ such that $I
\le I'$, $L' = H \cup I'$ and $\G \TH T \in \oTY$ such that if $F$ has
a non-neutral occurrence in $T$ then $F \in \FC$ and $F \le C$. Then,
one can prove by induction on $T$ that :

\begin{lst}{--}
\item if $\pos(C,T) \sle \pp(T)$ then $\JGT\Dtx[L \cup J^L] \le
  \JGT\Dtx[L' \cup J^{L'}]$,
\item if $\pos(C,T) \sle \pm(T)$ then $\JGT\Dtx[L \cup J^L] \ge
  \JGT\Dtx[L' \cup J^{L'}]$.
\end{lst}

~

Hence, $\vp^C$ has a least fixpoint. This gives us an interpretation
$I$ for all free predicate symbols. In the following, we let
$\JGT\Dtx[J] = \JGT\Dtx[I \cup J^I]$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% definition of the interpretation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\JGlr}[1]{\J{\Glr}{#1}}

\renewcommand{\Dtx}[1][J]{_{\D,\t,\xi}^{#1}}
\renewcommand{\Dspxp}[1][J]{_{\D,\s',\xi'}^{#1}}
\renewcommand{\Dstxp}[1][J]{_{\D,\s\t,\xi'}^{#1}}
\renewcommand{\Dspxpp}[1][J]{_{\D,\s',\xi''}^{#1}}
\renewcommand{\Dptx}[1][J]{_{\D',\t,\xi\Dp}^{#1}}
\renewcommand{\Dptpx}[1][J]{_{\D',\t',\xi\Dp}^{#1}}
\renewcommand{\Dpptpx}[1][J]{_{\D'',\t',\xi\Dpp}^{#1}}

\begin{dfn}[Valid interpretations]
  An interpretation $J$ for defined predicate symbols is {\em valid\,}
  if, for all $l\a r \in \cR_\FD$, $\JG{l\s}\Dtx = \JG{r\s}\Dtx$
  whenever $l\s\t \in \SN$.
\end{dfn}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% invariance by conversion
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The following property is essential for dealing with the type
conversion case.

\begin{lem}[Invariance by conversion]
  If $J$ is valid, $T \ad^* T'$ and $T\t, T'\t \in \SN$ then $\JGT\Dtx
  = \JGTp\Dtx$.
\end{lem}














%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% interpretation of defined predicate symbols

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Interpretation of defined predicate symbols}
\label{subsec-def}

In this subsection, we assume given an interpretation $I$ for free
predicate symbols and define an interpretation $J^I$ for defined
predicate symbols.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% basic rewrite system
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Basic rewrite systems}

\begin{dfn}
$J\DF = \top\DF$.
\end{dfn}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% positive rewrite system
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Positive rewrite systems}

Let $\cJ$ be the set of interpretations for all $F \in \FD$ and $\le$
be the relation on $\cJ$ defined by $J \le J'$ iff, for all $F \in
\FD$ and $\D$, $J\DF \le\DF J'\DF$. $(\cJ,\le)$ is a complete lattice.

\begin{dfn}
  Let $\psi$ be the function on $\cJ$ defined by :

\noindent
$\psi^J\DF(\va) =
\left\{
\begin{array}{l}
\JG{r}_{\D_n,\s,\xi}^J
\begin{array}[t]{l}
\mbox{ if } \vt \a^* \vl\s \in \NF\\
\mbox{ and } F(\vl) \a r \in \cR\\
\end{array}\\
\top_{\D_n \th F(\vt)} \mbox{ otherwise}\\
\end{array}
\right.$

\noindent
where $\G = \G_{F(\vl) \a r}$ and, for all $X \in \FVB(r)$, $X\xi =
S_{\k_X}\Dn$.
\end{dfn}

As for the interpretation of free predicate symbols, thanks to the
positivity condition, we can prove that $\psi$ is monotone. So, we
can let $J$ be the least fixpoint of $\psi$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% recursive rewrite system
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Recursive rewrite systems}

\begin{dfn}
  We define $J_F(\va)$ by induction on $F$ with $>_\cF$ as
  well-founded ordering and by induction on $\vt$ with $\tgt\sF$ as
  well-founded ordering :

\noindent
$J\DF(\va) =
\left\{
\begin{array}{l}
\JG{r}_{\D_n,\s,\xi}^J
\begin{array}[t]{l}
\mbox{ if } \vt \a^* \vl\s \in \NF\\
\mbox{ and } F(\vl) \a r \in \cR\\
\end{array}\\
\top_{\D_n \th F(\vt)} \mbox{ otherwise}\\
\end{array}
\right.$

\noindent
where $\G = \G_{F(\vl) \a r}$ and, for all $X \in \FVB(r)$, $X\xi
= S_{\k_X}\Dn$.
\end{dfn}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% validity
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Validity}

It is not difficult to see that the interpretation for basic types is
simply $\top$. As a consequence, the interpretation of the symbols
that belong to a basic rewrite system is valid. For the symbols in a
simple and positive or simple and recursive system, we use the fact
that the arguments of the left-hand side are free.













%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 



==> sn.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% strong normalization proof

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\Dtx}{_{\D,\t,\xi}}
\renewcommand{\Dsx}{_{\D,\s,\xi}}
\renewcommand{\Dspxp}{_{\D,\s',\xi'}}
\renewcommand{\Dsxp}{_{\D,\s,\xi'}}
\renewcommand{\Dtxp}{_{\D,\t,\xi'}}
\renewcommand{\Dstxp}{_{\D,\s\t,\xi'}}
\renewcommand{\Dspxpp}{_{\D,\s',\xi''}}
\renewcommand{\Dptx}{_{\D',\t,\xi\Dp}}
\renewcommand{\Dptpx}{_{\D',\t',\xi\Dp}}
\renewcommand{\Dpptpx}{_{\D'',\t',\xi\Dpp}}

\subsection{Strong normalization proof}
\label{subsec-sn}

We proceed in three steps. First, we prove the correctness of the
notions of accessibility and computable closure. Second, we prove the
reducibility of first-order and higher-order symbols. Finally, we
prove that every term belongs to the interpretation of its type. The
proofs of these results are close to the ones given in
\cite{blanqui99rta} or in \cite{jouannaud97tcs}. We only mention the
important differences. Full proofs can be found in \cite{blanqui00tr}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% accessibility correctness
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lem}[Accessibility correctness]
\label{lem-acc-correct}
If $\G \th u : U$, $\G \th t : T$, $u \in \acc(t)$ and $\D \TH t\t \in
\JGT\Dtx$ then $\D \TH u\t \in \JGU\Dtx$.
\end{lem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% definition of correct substitutions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{dfn}[Correct substitutions]
  Let $\t : \G \a \D$ and $\xi$ compatible with $(\t,\G,\D)$. $\t$ is
  {\em correct w.r.t. $\xi$} if, for all $x \in \dom(\G), \D \th x\t
  \in \JG{x\G}\Dtx$.
\end{dfn}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% computable closure correctness
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lem}[Computable closure correctness]
\label{lem-cc-correct}
Let $f \in \F$ with $\tf = \pvxT V$, $l \a r \in \cR$ with $l =
f(\vl)$, $\g = \vxl$, $\D$, $\s : \Glr \a \D$ and $\xi$ compatible
with $(\s,\Glr,\D)$. Assume that :

\begin{lst}{--}
\item $\s$ is correct w.r.t. $\xi$,
\item for all $i$, $\D \TH l_i\s \in \JGlr{T_i\g\r}\Dsx$,
\item for all $g \le_\cF f$, if $\tg = \pvyU W$, $\G' = \vy:\vU$ and
  $\t = \vyu$ is a well-typed substitution from $\G'$ to $\D$ correct
  w.r.t. some $\xi'$ compatible with $(\t,\G',\D)$ then $\D \TH g(\vu)
  \in \JGp{W}\Dtxp$ whenever $g <_\cF f$ or $\vu \tlt\sf \vl\s$.
\end{lst}

\noindent
Then, $\D \TH r\s \in \JGlr{V}\Dsx$.
\end{lem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% reducibility of first-order symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lem}{\bf(Reducibility of first-order symbols)}
\label{lem-symb-fo-red}
Let $f \in \Fu$ with $\tf = \pvxT U$, $\G' = \vx:\vT$, $\D \in \E$,
$\t : \G' \a \D$ and $\xi$ compatible with $(\t,\G',\D)$. If $\t$ is
correct w.r.t. $\xi$ then $\D \TH f(\vx\t) \in \JGpU\Dtx$.
\end{lem}

By assumption on $\Fu$, $f$ is either a predicate symbol or the
constructor of some basic predicate symbol. Thus, $\JGpU\Dtx =
\oSN\DUt$ and, since $\t$ is correct w.r.t. $\xi$, it suffices to
prove that every immediate reduct of $f(\vx\t)$ is strongly
normalizable, even if $f$ is a constructor. This can be done as in
\cite{jouannaud97tcs}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% reducibility of higher-order symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lem}{\bf(Reducibility of higher-order symbols)}
\label{lem-symb-ho-red}
Let $f \in \Fw$ with $\tf = \pvxT U$, $\G' = \vx:\vT$, $\D$, $\t : \G'
\a \D$ and $\xi$ compatible with $(\t,\G',\D)$. If $\t$ is correct
w.r.t. $\xi$ then $\D \TH f(\vx\t) \in \JGpU\Dtx$.
\end{lem}

\begin{prf}
  Let $t_i = x_i\t$ and $t=f(\vt)$. As in \cite{blanqui99rta}, we
  prove the lemma by induction on $(f,\vt)$ with $(>_\cF, (\a \!\cup
  \,\tgt)\sf)\lex$ as well-founded ordering.
  
  We saw in the previous lemma that it suffices to prove that, for
  every immediate reduct $t'$ of $t$, $\D \TH t' \in \JGpU\Dtx$, even
  if $f$ is a constructor. The delicate point is when there are a rule
  $l \a r$ with $l = f(\vl)$ and a substitution $\s$ such that $\vt =
  \vl\s$. From the assumptions on rewrite rules, the property (A3) and
  the Candidate substitution Lemma, we can define a candidate
  assignment $\xi'$ such that $\JGpU\Dtx = \JGlr{U\g\r}\Dsxp$. By
  Accessibility correctness, we can prove that $\s$ is correct w.r.t
  $\xi'$ and, then, apply the Computable closure correctness Lemma.
\end{prf}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% main lemma for strong normalization
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lem}[Main lemma]
  For every $\G \th t : T$, $\D$, $\t : \G \a \D$, $\xi$ compatible
  with $(\t,\G,\D)$, if $\t$ is correct w.r.t. $\xi$ then $\D \TH t\t
  \in \JGT\Dtx$.
\end{lem}

The proof, by induction on $\G \th t:T$, is the same as for the
Computable closure correctness Lemma. The symbol cases are treated by
the previous lemmas and the conversion case is due to the invariance
by conversion of the interpretation.

Then, we get the strong normalization that taking the identity and the
candidate assignment $x\xi = \top_{\G \th x\t}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% strong normalization theorem
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{thm}[Strong normalization]
  In an admissible CAC, every typable term is strongly normalizable.
\end{thm}








%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

